Neural Mutual Information Estimation with Vector Copulas

Estimating mutual information (MI) is a fundamental task in data science and machine learning. Existing estimators mainly rely on either highly flexible models (e.g., neural networks), which require large amounts of data, or overly simplified models (e.g., Gaussian copula), which fail to capture complex distributions. Drawing upon recent vector copula theory, we propose a principled interpolation between these two extremes to achieve a better trade-off between complexity and capacity. Experiments on state-of-the-art synthetic benchmarks and real-world data with diverse modalities demonstrate the advantages of the proposed estimator.

==> figs_and_tables/figs_n_components.tex <==
\begin{figure*}[t!]
            %\vspace{0.35cm}
            \hspace{-0.005\linewidth}
            \begin{subfigure}{.245\textwidth}
            %\subfigure[\centering Rectangles]{
                    \centering
                    % \label{fig:rectangles}
                    \begin{minipage}[t]{1.0\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_rectangle_MI.png}
                    \end{minipage}
            %}
            \end{subfigure}
            \hspace{-0.0125\linewidth}
            \begin{subfigure}{.245\textwidth}
            %\subfigure[\centering Gaussian plates]{
                    \centering
                    % \label{fig:gaussians}
                    \begin{minipage}[t]{1.0\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_gaussian_MI.png}
                    \end{minipage}
            %}
            \end{subfigure}
            \hspace{-0.0125\linewidth}
            \begin{subfigure}{.245\textwidth}
            %\subfigure[\centering MoG]{
                    \centering
                    % \label{fig:gaussians}
                    \begin{minipage}[t]{1.0\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_MoG_MI.png}
                    \end{minipage}
            %}
            \end{subfigure}
            \hspace{-0.0125\linewidth}
            \begin{subfigure}{.245\textwidth}
            %\subfigure[\centering BERT]{
                    \centering
                    % \label{fig:gaussians}
                    \begin{minipage}[t]{1.0\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_bert_MI.png}
                    \end{minipage}
            %}
            \end{subfigure}
\caption{Exploring the effect of number of components $K$ in the vector copula density $c$ in VCE. }
\label{fig:number-of-component-K}
\end{figure*}


\if0
\begin{figure*}[t!]
            %\vspace{0.35cm}
            \hspace{-0.005\linewidth}
            \subfigure[\centering Rectangles]{
                    \centering
                    % \label{fig:rectangles}
                    \begin{minipage}[t]{0.24\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_rectangle_MI.png}
                    \end{minipage}
            }
            \hspace{-0.015\linewidth}
            \subfigure[\centering Gaussian plates]{
                    \centering
                    % \label{fig:gaussians}
                    \begin{minipage}[t]{0.24\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_gaussian_MI.png}
                    \end{minipage}
            }
            \hspace{-0.015\linewidth}
            \subfigure[\centering MoG]{
                    \centering
                    % \label{fig:gaussians}
                    \begin{minipage}[t]{0.24\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_MoG_MI.png}
                    \end{minipage}
            }
            \hspace{-0.015\linewidth}
            \subfigure[\centering BERT]{
                    \centering
                    % \label{fig:gaussians}
                    \begin{minipage}[t]{0.24\linewidth}
                    \centering
                     \includegraphics[width=1.0\linewidth]{figures/K_components/K_components_bert_MI.png}
                    \end{minipage}
            }
\caption{Exploring the effect of number of components $K$ in the vector copula density $c$ in our VCE method. }
\label{fig:number-of-component-K}
\end{figure*}
\fi

==> figs_and_tables/table_joint_vs_separate.tex <==
\begin{table*}[t]
  % \label{acceleration}
\centering
\hspace{0.00\textwidth}
%\subfigure[Joint training]{
\begin{subfigure}{0.495\textwidth}
\begin{minipage}{1.0\textwidth}
 \begin{tabular}{lcccc}
    \toprule
    \cmidrule(r){1-5}
	& median	& std	& fail*	& $I_{\text{truth}}$ \\
\midrule
Student-$t$	& 7.81 & 5.55 & 2/10 & 12.4	 \\
   \midrule
$\mathbf{A}X^3, \mathbf{B}e^Y$	& 6.02 & 0.98 & 1/10 & 10.8		 \\
    \bottomrule \\
  \end{tabular}
\end{minipage}
%}
\subcaption{Joint learning}
\end{subfigure}
\hspace{-0.01\textwidth}
%\subfigure[Separate learning]{
\begin{subfigure}{0.495\textwidth}
\begin{minipage}{1.0\textwidth}
 \begin{tabular}{lcccc}
    \toprule
    \cmidrule(r){1-5}
	& median	& std	& fail*	& $I_{\text{truth}}$ \\
\midrule
Student-$t$	& 9.50 & 0.35 & 0/10 & 12.4	 \\
   \midrule
$\mathbf{A}X^3, \mathbf{B}e^Y$	& 8.12 & 0.12 & 0/10 & 10.8		 \\
    \bottomrule \\
  \end{tabular}
\end{minipage}
%}
\subcaption{Separate learning}
\end{subfigure}
\caption{Joint learning vs separate learning. Results are collected from 8 independent runs. Data dimensionality is 64. *Fail: fraction of independent runs where $|\hat{I}(X; Y) - I(X; Y)| > \frac{1}{2}I(X; Y)$. }
\label{tab:joint-vs-separate-1}
\end{table*}




\if0
\begin{table*}[t]
  % \label{acceleration}
\centering
\hspace{0.00\textwidth}
\begin{subfigure}{0.495\textwidth}
%\subfigure[Joint training]{
\begin{minipage}{1.0\textwidth}
 \begin{tabular}{lccc}
    \toprule
    \cmidrule(r){1-4}
	& $t_{\text{marginal}}$	& $t_{\text{copula}}$	& $t_{\text{overall}}$ 	  \\
\midrule
Student-$t$	& - & - & 163.4 	 \\
   \midrule
$\mathbf{A}X^3, \mathbf{B}e^Y$	& - & - & 156.7   		 \\
    \bottomrule \\
  \end{tabular}
        \centering{Computational complexity: $\mathcal{O}(Nt_{\text{overall}})$}
\end{minipage}
%}
\end{subfigure}
\hspace{-0.01\textwidth}
\begin{subfigure}{0.495\textwidth}
%\subfigure[Separate learning]{
\begin{minipage}{1.0\textwidth}
 \begin{tabular}{lccc}
        \toprule
    \cmidrule(r){1-4}
	& $t_{\text{marginal}}$	& $t_{\text{copula}}$	& $t_{\text{overall}}$ 	  \\
\midrule
Student-$t$	& 75.3 & 58.9 & 134.2 	 \\
   \midrule
$\mathbf{A}X^3, \mathbf{B}e^Y$	& 79.8 & 44.5 & 124.3  		 \\
    \bottomrule \\
  \end{tabular}
      \centering{Computational complexity: $\mathcal{O}(t_{\text{marginal}} + Nt_{\text{copula}})$}
\end{minipage}
%}
\end{subfigure}
\caption{Execution time comparison (secs). $N =$ the number of models needed to be trained in model selection.}
\end{table*}
\fi







\if0
\begin{table*}[t]
  % \label{acceleration}
\centering
\hspace{0.00\textwidth}
\subfigure[Joint training]{
\begin{minipage}{0.485\textwidth}
 \begin{tabular}{lcccc}
    \toprule
    \cmidrule(r){1-5}
	& median	& std	& fail*	& $I(X; Y)$ \\
\midrule
Student-$t$ ($\nu = 1$)	& 7.81 & 5.55 & 2/10 & 12.4	 \\
   \midrule
$\mathbf{A}X^3, \mathbf{B}e^Y$	& 6.02 & 0.98 & 1/10 & 10.8		 \\
    \bottomrule \\
  \end{tabular}
\end{minipage}
}
%\hspace{-0.01\textwidth}
\subfigure[Separate learning]{
\begin{minipage}{0.485\textwidth}
 \begin{tabular}{lcccc}
    \toprule
    \cmidrule(r){1-5}
	& median	& std	& fail*	& $I(X; Y)$ \\
\midrule
Student-$t$ ($\nu = 1$)	& 9.50 & 0.35 & 0/10 & 12.4	 \\
   \midrule
$\mathbf{A}X^3, \mathbf{B}e^Y$	& 8.12 & 0.12 & 0/10 & 10.8		 \\
    \bottomrule \\
  \end{tabular}
\end{minipage}
}
*Fail: fraction of runs where $|\hat{I}(X; Y) - I(X; Y)| > \frac{1}{2}I(X; Y)$.
\caption{Some failure case of joint learning. All results correspond to 10 independent runs. Data dimensionality is 64.  }
\end{table*}
\fi
